A parallel space-time multigrid method for the eddy-current equation

We expand the applicabilities and capabilities of an already existing space-time parallel method based on a block Jacobi smoother. First we formulate a more detailed criterion for spatial coarsening, which enables the method to deal with unstructured meshes and varying material parameters. Further we investigate the application to the eddy-current equation, where the non-trivial kernel of the curl operator causes severe problems. This is remedied with a new nodal auxiliary space correction. We proceed to identify convergence rates by local Fourier analysis and numerical experiments. Finally, we present a numerical experiment which demonstrates its excellent scaling properties.

==> Makefile <==
filepre = thesis

texfile = $(filepre).tex
dvifile = $(filepre).dvi

editobjs = header.tex \
	frontpage.tex frontmatter.tex \
	bibliography.tex \
	problem.tex discretization.tex \
	mgnewt.tex conclusion.tex  \
	numerics.tex introduction.tex

dvi:
	latex $(texfile); latex $(texfile); latex $(texfile)

update:
	latex $(texfile)

edit:
	xemacs $(texfile) $(editobjs)&

view:
	kdvi $(dvifile) &

ps: dvi
	dvips -P cmz $(dvifile) -o $(filepre).ps

pdf: dvi
	dvips -P pdf $(dvifile) -o $(filepre).ps.temp && \
	ps2pdf $(filepre).ps.temp $(filepre).pdf

tar:
	tar -cf cds.tar Makefile *.tex *.eps *.sty

clean:
	rm -f *~ *.aux *.log *.toc


==> bibliography.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% bibliography.tex
% 
% Bibliography
%
% Diploma Thesis
% (c) 2003/04 Clemens Pechstein
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{thebibliography}{99}
\addcontentsline{toc}{chapter}{Bibliography} 

\bibitem{Neum}
M. Neum\"{u}ller,
\emph{Space-Time Methods, Fast Solvers and Applications}.
Dissertation, Graz University of Technology, Institute of Computational Mathematics, 2013

\bibitem{Master}
M. Schwalsberger,
\emph{A Space-Time Parallel Multigrid Method for the Transient Eddy-Current Equation}
Master thesis, JKU Linz, Institut f\"ur Numerische Mathematik, November 2018

\bibitem{Hiptmayr}
R. Hiptmayr, 
\emph{Multigrid Method for Maxwell's Equation}, 
SIAM J. NUMER. ANAL., Vol. 36, No. 1, pp. 204-225, 1998

\bibitem{GanderNeum}
M. Gander, M. Neum\"{u}ller, 
\emph{Analysis of a New Space-Time Parallel Multigrid Algorithm for Parabolic Problems}
SIAM J. Sci. Comput., 38(4), A2173-A2208, JULY 2016

\bibitem{Zaglmayr}
S. Zaglmayr, 
\emph{High Oder Finite Element Methods for Electromagnetic Field Computation}
Dissertation, JKU Linz, Institut f\"ur Numerische Mathematik, 2006

%\bibitem{EddyBuch}
%A. Rodr\'{\i}guez, A. Valli,
%\emph{Eddy Current Approximation of Maxwell Equations}.
%Springer Verlag, 2010

%\bibitem{ModelError}
%K. Schmidt, O. Sterz, R. Hiptmair,
%\emph{Estimating the Eddy-Current Modeling Error}.
%IEEE TRANSACTIONS ON MAGNETICS, VOL. 44, NO. 6, JUNE 2008

%\bibitem{EddyRegu}
%F. Bachinger, U. Langer, and J. Sch\"oberl,
%\emph{Numerical Analysis of Nonlinear Multiharmonic Eddy Current Problems}.
%Numerische Mathematik. 100(4), 594-616, 2005 

\bibitem{Monk}
P. Monk,
\emph{Finite Element Methods for Maxwell's Equation}.
Clarendon Press, Oxford 2003 

%\bibitem{WikiInd}
%English Wikipedia links:
%\emph{https://en.wikipedia.org/wiki/Induction\_furnace},
%May 2018

%\bibitem{WikiConst}
%English Wikipedia links:\newline
%\emph{https://en.wikipedia.org/wiki/Electrical\_resistivity\_and\_conductivity}\newline
%\emph{https://en.wikipedia.org/wiki/Permeability\_(electromagnetism)},
%May 2018

\bibitem{EddyFourier}
T. Boonen, J. van Lent, S.Vandewalle,
\emph{Local Fourier Analysis of Multigrid for the Curl-Curl Equation}.
Siam J. SCI. COMPUT. Vol. 30, pp. 1730-1755


\bibitem{AllgemeinFourier}
U. Trottenberg, C. Oosterlee, A.Sch\"uller,
\emph{Multigrid},
Academic Press, December 2000

\bibitem{Software}
MFEM, 
\emph{http://mfem.org/}~~
January 2018

%\bibitem{glvis}
%GLVIS, 
%\emph{http://glvis.org/}~~
%January 2018

\bibitem{hypre}
HYPRE, 
\emph{https://computation.llnl.gov/projects/hypre-scalable-linear-solvers-multigrid-methods}~~
January 2018

%\bibitem{Netgen}
%Netgen,
%\emph{https://ngsolve.org/}~~
%December 2017

\bibitem{Mathematica}
Mathematica 10 by Wolfram, 
\emph{https://www.wolfram.com/mathematica/}

\bibitem{50Years}
M. Gander, 
\emph{50 Years of Time Parallel Time Integration},
Springer Verlag, 2015

\bibitem{NeumStoch}
M. Neum\"{u}ller, A. Thalhammer,
\emph{A Fully Parallelizable Space-Time Multilevel Monte Carlo Method for Stochastic Differential Equations with Additive Noise},
SIAM J. Sci. Comput., 40(3), C388-C400, 2018

%\bibitem{Wessel}
%P. Wesseling,
%\emph{An Introduction to Multigrid Methods},
%John Wiley \& Sons Ltd., 1992. Corrected Reprint. Philadelphia: R.T. Edwards, Inc., 2004.



\bibitem{STMG}
G. Horton, S. Vandewalle, 
\emph{A Space-Time Multigrid Method for Parabolic Partial Differential Equations},
SIAM J. Sci. Comput., Vol. 16, No. 4, pp. 848-864, July 1995

\bibitem{NeumIsogeometric}
C. Hofer, U. Langer, M. Neum\"uller and I. Toulopoulos, 
\emph{Time-Multipatch Discontinuous Galerkin Space-Time Isogeometric Analysis of Parabolic Evolution Problems}.
Electronic Transactions on Numerical Analysis (ETNA) 49, 126-150, 2018

\bibitem{First!}
J. Nievergelt, 
\emph{Parallel methods for integrating ordinary differential equations}.
Commun. ACM 7, 731-733 (1964)

\bibitem{WRMG-CR}
Horton, G., Vandewalle, S., Worley, P.: 
\emph{An algorithm with polylog parallel complexity for solving parabolic partial differential equations}.
SIAM J. Sci. Comput. 16 (3), 531-541 (1995)

\bibitem{MGRIT}
Falgout, R.D., Friedhoff, S., Kolev, T.V., MacLachlan, S.P., Schroder, J.B.: 
\emph{Parallel time integration with multigrid}. 
SIAM J. Sci. Comput. 36 (6), C635-C661 (2014)

\bibitem{MGRIT2}
R.D. Falgout, S. Friedhoff, Tz.V. Kolev, S.P. MacLachlan, J.B. Schroder and S. Vandewalle, 
\emph{Multigrid Methods with Space-Time Concurrency},
 Computing and Visualization in Science, Springer, (2017).

\bibitem{MGRIT3}
V. Dobrev, Tz. Kolev, N. A. Petersson, and J. B. Schroder, 
\emph{Two-level convergence theory for Multigrid Reduction in Time (MGRIT)},
 SIAM J. Sci. Comput., 39 (2017), pp. 501-527

\bibitem{MGRIT4}
R. D. Falgout, T. A. Manteuffel, B. O'Neill, and J. B. Schroder, 
\emph{Multigrid reduction in time for nonlinear parabolic problems: A Case Study},
 SIAM J. Sci. Comput., 39 (2017), pp 298-322

\bibitem{MGRIT5}
M. Lecouvez, R. D. Falgout, C. S. Woodward, and P. Top, 
\emph{A parallel multigrid reduction in time method for power systems},
 in Power and Energy Society General Meeting (PESGM), 2016, IEEE, 2016, pp. 1–5.

\bibitem{MGRIT6}
H. Gahvari, V. A. Dobrev, R. D. Falgout, Tz. V. Kolev, J. B. Schroder, M. Schulz and U. M. Yang, 
\emph{A Performance Model for Allocating the Parallelism in a Multigrid-in-Time Solver},
 The 7th International Workshop on Performance Modeling, Benchmarking and Simulation of High Performance Computer Systems (PMBS16), Supercomputing 16.

\bibitem{MGRIT7}
S. Gunther, N. R. Gauger, and J. B. Schroder, 
\emph{A Non-Intrusive Parallel-in-Time Adjoint Solver with the XBraid Library},
 Computing and Visualization in Science, Springer, (2018). 

\bibitem{MGRIT8}
J. B. Schroder, M. Lecouvez, R. D. Falgout, C. S. Woodward, P. Top, 
\emph{Parallel-in-Time Solution of Power Systems with Scheduled Events},
 2018 Power and Energy Society General Meeting (PESGM), IEEE, (2018).

\bibitem{VandewalleTeubner}
S. Vandewalle,
\emph{Parallel Multigrid Waveform Relaxation for Parabolic Problems.} 
Teubner Skripten zur Numerik. Vieweg+Teubner Verlag  (1993) 

\bibitem{LubichOstermann}
C. Lubich, A. Ostermann,
\emph{Multi-grid dynamic iteration for parabolic equations},
BIT, 27 (1987), pp. 216-234.

\bibitem{Hackbusch1984}
W. Hackbusch,
\emph{Parabolic multi-grid methods},
Computing Methods in Applied Sciences and Engineering, VI, R. Glowinski and J.-L. Lions, eds., North-Holland, 1984, pp. 189-197.

\bibitem{Aachen1}
 R. Speck, D. Ruprecht, R. Krause, M. Emmett, M. Minion, M. Winkel, P. Gibbon,
\emph{A massively space-time parallel N-body solver}
IEEE Computer Society Press 11 p. (2012).

\bibitem{Aachen2}
R. Speck, D. Ruprecht, M. Emmett, M. Minion, M. Bolten, R. Krause,
\emph{A space-time parallel solver for the three-dimensional heat equation}
IOS Press, Advances in Parallel Computing 25, 263 - 272 (2014).

\bibitem{Aachen3}
R. Speck, D. Ruprecht, R. Krause, M. Emmett, M. Minion, M. Winkel, P. Gibbon,
\emph{Integrating an N-Body Problem with SDC and PFASST}
Springer International Publishing, Lecture Notes in Computational Science and Engineering 98, 637 - 645 (2014).

\bibitem{Aachen4}
R. Speck, D. Ruprecht, M. Emmett, M. Minion, M. Bolten, R. Krause,
\emph{A multi-level spectral deferred correction method}
BIT 55(3), 843-867 (2015) 

\bibitem{Aachen5}
J. Steiner, D. Ruprecht, R. Speck, R.  Krause,
\emph{Convergence of Parareal for the Navier-Stokes Equations Depending on the Reynolds Number}
Cham : Springer International Publishing, Lecture Notes in Computational Science and Engineering 103, 195 - 202 (2015)

\bibitem{Aachen6}
M. Winkel, R. Speck, D. Ruprecht,
\emph{A high-order Boris integrator}
Journal of computational physics 295, 456 - 474 (2015)

\bibitem{Aachen7}
D. Ruprecht, R. Speck, R. Krause,
\emph{Parareal for diffusion problems with space- and time-dependent coefficients}
Springer International Publishing Switzerland, Lecture Notes in Computational Science and Engineering 104, 3-10 (2015)

\bibitem{Aachen8}
R. Speck, D. Ruprecht, M. Minion, M. Emmett, R. Krause,
\emph{Inexact spectral deferred corrections}
Springer International Publishing Switzerland, Lecture Notes in Computational Science and Engineering 104, 127-133 (2015)

\bibitem{Aachen9}
M. Minion, R. Speck, M. Bolten, M. Emmett, D. Ruprecht,
\emph{Interweaving PFASST and Parallel Multigrid}
SIAM journal on scientific computing 37(5), S244 - S263 (2015)

\bibitem{Aachen10}
A. Kreienbuehl, A. Naegel, D. Ruprecht, R. Speck, G. Wittum, R. Krause,
\emph{Numerical simulation of skin transport using Parareal}
Computing and visualization in science 17(2), 99 - 108 (2015)

\bibitem{Aachen11}
D. Ruprecht, R. Speck,
\emph{Spectral Deferred Corrections with Fast-wave Slow-wave Splitting}
SIAM journal on scientific computing 38(4), A2535 - A2557 (2016)

\bibitem{Aachen12}
R. Speck, D. Ruprecht,
\emph{Toward fault-tolerant parallel-in-time integration with PFASST}
Parallel computing 62, 20 - 37 (2017)

\bibitem{Aachen13}
M. Bolten, D. Moser, R. Speck,
\emph{A multigrid perspective on the parallel full approximation scheme in space and time}
Numerical linear algebra with applications 24(6), e2110 (2017)

\bibitem{Aachen14}
R. Speck,
\emph{Parallelizing spectral deferred corrections across the method}
Computing and visualization in science 19(3-4), 75-83 (2018)

\bibitem{Aachen15}
M. Bolten, D. Moser, R. Speck,
\emph{Asymptotic convergence of the parallel full approximation scheme in space and time for linear problems}
Numerical linear algebra with applications 25(6), e2208 - (2018) 

\bibitem{Aachen16}
R. Speck,
\emph{Algorithm 997: pySDC - Prototyping Spectral Deferred Corrections}
ACM transactions on mathematical software 45(3), 35 (2019)


\end{thebibliography}

% EOF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

